Real-Time Personalization for LLM-based Recommendation with Customized In-Context Learning

Frequently updating Large Language Model (LLM)-based recommender systems to adapt to new user interests -- as done for traditional ones -- is impractical due to high training costs, even with acceleration methods. This work explores adapting to dynamic user interests without any model updates by leveraging In-Context Learning (ICL), which allows LLMs to learn new tasks from few-shot examples provided in the input. Using new-interest examples as the ICL few-shot examples, LLMs may learn real-time interest directly, avoiding the need for model updates. However, existing LLM-based recommenders often lose the in-context learning ability during recommendation tuning, while the original LLM's in-context learning lacks recommendation-specific focus. To address this, we propose RecICL, which customizes recommendation-specific in-context learning for real-time recommendations. RecICL organizes training examples in an in-context learning format, ensuring that in-context learning ability is preserved and aligned with the recommendation task during tuning. Extensive experiments demonstrate RecICL's effectiveness in delivering real-time recommendations without requiring model updates. Our code is available at https://github.com/ym689/rec_icl.

==> table/bin_tall_ICL_decrease.tex <==
% \begin{table*}[ht]
%     \centering

%     \begin{tabular}{c|c|cc|cc|cc}
%     \hline
%     & \multicolumn{1}{c|}{Model}                     & \multicolumn{2}{c|}{TALLRec}               & \multicolumn{2}{c|}{BinLLM}     & \multicolumn{2}{c}{General LLM}   \\ \hline
%     & \multicolumn{1}{c|}{Setting}                   & $\mathcal{D}_{5}$    & $\mathcal{D}_{9}$             & $\mathcal{D}_{5}$    & $\mathcal{D}_{9}$ & $\mathcal{D}_{5}$    & $\mathcal{D}_{9}$    \\ \hline
%    \multicolumn{1}{c|}{\multirow{3}{*}{Amazon-Book}} & \multicolumn{1}{c|}{Without Incontext}         & 0.7335          & 0.7005                   & 0.7936          & 0.7787       & 0.6085          & 0.5637               \\ \hline
%   \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{With Incontext}            & 0.7495          & 0.7290                   & 0.7813          & 0.7708       & 0.7162          & 0.7133        \\ \hline
%     % \multicolumn{1}{c|}{Random Incontext}          & 0.6514          & 0.6369                   & 0.6958          & 0.5969       & 0.5029          & 0.5025        \\ \hline
%     % \hline
%     \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{Imp}                  & 0.0160          & 0.0285                   & -0.0123          & -0.0079       &\textbf{0.1077 }             & \textbf{0.1400 }         \\
%     \hline
%     & \multicolumn{1}{c|}{Without Incontext}         & 0.7927          & 0.7415                   & 0.8108          & 0.7658       & 0.6416          & 0.6078               \\ \hline
%     & \multicolumn{1}{c|}{With Incontext}            & 0.7424          & 0.6712                   & 0.8285          & 0.7835       & 0.7511          & 0.7522        \\ \hline
%     & \multicolumn{1}{c|}{Imp}                  & -0.0503          & -0.0703                   & 0.0177          & 0.0177       &\textbf{0.1095 }             & \textbf{0.1444 }         \\
%     \hline
%     \end{tabular}
%         \caption{The performance of TALLRec BinLLM and General LLM in scenarios with and without in-context learning. The last row of the table shows the performance improvement brought by using in-context learning. Here in-context learning refers to we \bkq{select four most-recent interactions for each user to formulate the few-shot examples.}
% }
%     \label{pre_exp}
% \end{table*}
\begin{table*}[ht]
    \centering
    \caption{Performance of TALLRec, BinLLM, and General LLM in scenarios with and without in-context learning. The "Imp" row shows the performance improvement brought by using in-context learning, where in-context learning refers to selecting the four most recent interactions for each user to formulate the few-shot examples.}
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{} & \multirow{2}{*}{Setting} & \multicolumn{2}{c|}{TALLRec} & \multicolumn{2}{c|}{BinLLM} & \multicolumn{2}{c}{General LLM} \\ \cline{3-8}
                      &                          & $\mathcal{D}_{5}$ & $\mathcal{D}_{9}$ & $\mathcal{D}_{5}$ & $\mathcal{D}_{9}$ & $\mathcal{D}_{5}$ & $\mathcal{D}_{9}$ \\ \hline
    \multirow{3}{*}{Amazon-Book} & Without Incontext & 0.7335 & 0.7005 & 0.7936 & 0.7787 & 0.6085 & 0.5637 \\ \cline{2-8}
                                & With Incontext    & 0.7495 & 0.7290 & 0.7813 & 0.7708 & 0.7162 & 0.7133 \\ \cline{2-8}
                                & Imp               & 0.0160 & 0.0285 & -0.0123 & -0.0079 & \textbf{0.1077} & \textbf{0.1400} \\ \hline
                                \midrule
    \multirow{3}{*}{Amazon-Movie} & Without Incontext & 0.7927 & 0.7415 & 0.8108 & 0.7658 & 0.6416 & 0.6078 \\ \cline{2-8}
                                    & With Incontext    & 0.7424 & 0.6712 & 0.8285 & 0.7835 & 0.7511 & 0.7522 \\ \cline{2-8}
                                    & Imp               & -0.0503 & -0.0703 & 0.0177 & 0.0177 & \textbf{0.1095} & \textbf{0.1444} \\ \bottomrule
    \end{tabular}
    
    \label{pre_exp}
\end{table*}


==> table/cold_warm.tex <==

\begin{table*}[ht]
    \centering
    \caption{Performance of TALLRec, BinLLM, and General LLM in scenarios with and without in-context learning. The "Imp" row shows the performance improvement brought by using in-context learning, where in-context learning refers to selecting the four most recent interactions for each user to formulate the few-shot examples.}
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{} & \multirow{2}{*}{Setting} & \multicolumn{1}{c|}{TALLRec} & \multicolumn{1}{c|}{BinLLM} & \multicolumn{1}{c}{General LLM} \\ \cline{3-8}
                      &                          & $\mathcal{D}_{5}$ & $\mathcal{D}_{9}$ & $\mathcal{D}_{5}$ & $\mathcal{D}_{9}$ & $\mathcal{D}_{5}$ & $\mathcal{D}_{9}$ \\ \hline
    \multirow{2}{*}{Amazon-Book} & Cold          & 0.7335 & 0.7005 & 0.7936 & 0.7787 & 0.6085 & 0.5637 \\ \cline{2-8}
                                
                                & Warm               & 0.0160 & 0.0285 & -0.0123 & -0.0079 & \textbf{0.1077} & \textbf{0.1400} \\ \hline
                                \midrule
    \multirow{2}{*}{Amazon-Movie} & Cold & 0.7927 & 0.7415 & 0.8108 & 0.7658 & 0.6416 & 0.6078 \\ \cline{2-8}
                                    
                                & Warm               & -0.0503 & -0.0703 & 0.0177 & 0.0177 & \textbf{0.1095} & \textbf{0.1444} \\ \bottomrule
    \end{tabular}
    
    \label{pre_exp}
\end{table*}


==> table/table_fewshot_template.tex <==
% \begin{table}
% % \small
% \centering

%     % \vspace{-10pt}
%  \label{tab:prompt-example}
%     \begin{tabular}{p{7.5cm}}  
%     \hline
%         #You are a smart book recommendation system that predicts whether a user will enjoy a book based on their preferences. Below are a few examples:\\#Example1 <$CS_\mathrm{1}$>,...,#ExampleN<$CS_\mathrm{N}$>,#IS\\
%     \hline
%     \end{tabular}
%       \caption{
%         Example of our few-shot template.
%     }
% \end{table}

==> table/table_sample_template.tex <==
% \begin{table}
% % \small
% \centering

%     \vspace{-1em}
%     \label{tab:prompt-example}
%     \begin{tabular}{p{7.5cm}}  
%     \hline
%         \#Question: A user has given high ratings to the following books: <ItemTitleList>. Leverage the information to predict whether the user would enjoy the book titled <TargetItemTitle>? Answer with "Yes" or "No". \#Answer:\\
%     \hline
%     \end{tabular}
%       \caption{
%         Example of the used prompt template.
%     }
% \end{table}
